Entanglement with neutral atoms in the simulation of nonequilibrium dynamics of one-dimensional spin models

Quantum entanglement is a key ingredient for quantum information processing with capabilities beyond that of classical computation. We study the generation and role of entanglement in the dynamics of spin-1/2 models, both for the design of quantum gates for general-purpose quantum computation and for quantum simulation of interacting spin models. We introduce the neutral atom M{\o}lmer-S{\o}rensen gate, involving rapid adiabatic Rydberg dressing interleaved in a spin-echo sequence. We show its robustness to quasi-static experimental imperfections and favorable scaling with the time-energy scales of Rydberg-mediated entanglement generation. In quantum simulation, we consider critical behavior in quench dynamics of transverse field Ising models. Using matrix product states to calculate the dynamics, we find that order parameters, critical point, and critical exponents can be estimated using modest bond dimensions. Considering the role of chaos and equilibration in quenches, we find that local observables are well approximated either due to low global entanglement or the proximity of local marginals to the maximally mixed state. These findings highlight the challenge of identifying relevant quantum phenomena that remain inaccessible to classical descriptions. Understanding the regimes where classical descriptions fail but remain accessible to pre-fault tolerant quantum hardware will help inform the design of future quantum information processors

==> frontmatter/abstract.tex <==
%%%%%% short abstract %%%%%
Quantum entanglement is a key ingredient for quantum information processing with capabilities beyond that of classical computation. We study the generation and role of entanglement in the dynamics of spin-1/2 models, both for the design of quantum gates for general-purpose quantum computation and for quantum simulation of interacting spin models. We introduce the neutral atom Mølmer-Sørensen gate, involving rapid adiabatic Rydberg dressing interleaved in a spin-echo sequence. We show its robustness to quasi-static experimental imperfections and favorable scaling with the time-energy scales of Rydberg-mediated entanglement generation. In quantum simulation, we consider critical behavior in quench dynamics of transverse field Ising models. Using matrix product states to calculate the dynamics, we find that order parameters, critical point, and critical exponents can be estimated using modest bond dimensions. Considering the role of chaos and equilibration in quenches, we find that local observables are well approximated either due to low global entanglement or the proximity of local marginals to the maximally mixed state. These findings highlight the challenge of identifying relevant quantum phenomena that remain inaccessible to classical descriptions. Understanding the regimes where classical descriptions fail but remain accessible to pre-fault tolerant quantum hardware will help inform the design of future quantum information processors

%%%%%% long abstract %%%%%
% Quantum entanglement is a key ingredient for quantum information processing with capabilities beyond that of classical computation. In this dissertation, we study the generation and role of entanglement in the dynamics of many-body spin-1/2 models, both for the design of quantum gates for general-purpose quantum computation and for quantum simulation of interacting spin models.

% We study the entanglement of neutral atoms using the adiabatic Rydberg dressing paradigm. We introduce the neutral atom Mølmer-Sørensen gate, involving rapid adiabatic Rydberg dressing passages interleaved in a spin-echo sequence. This allows for a separation of the one-qubit and two-qubit components of an entangling gate. We show that the fidelity of the gate is more sensitive to errors in the one-qubit component and that the spin-echo sequence corrects these errors, leading to a robust gate. Finally, we show that the adiabatic Rydberg dressing paradigm can be extended to regimes beyond the Rydberg blockade and can achieve the fundamental bounds of entanglement generation for neutral atoms using interactions between Rydberg states. The findings provide a path towards Rydberg-mediated entanglement between neutral atoms in future experiments in large arrays of atoms, and sufficient laser power to harness the interactions between Rydberg states.

% Quantum simulation is considered an application where quantum advantage can be achieved without fault-tolerant error correction. The dynamics of many-body quantum systems is a common paradigm in analog quantum simulation experiments with multiple interacting degrees of freedom. It is critical, however, to distinguish between the simulation of microstates versus macrostates. While tracking the exact many-body state of a quantum simulator may be intractable, this does not imply that the macro-properties we seek to extract cannot be efficiently simulated classically. We ask how well can the quantities based on macro-properties, like critical point and critical exponents of a phase transition, be simulated efficiently using classical methods. Using matrix product states to calculate the dynamics, we find that not only the order parameters but also the critical point and critical exponents can be estimated using modest bond dimensions. We also relate the approximation of local observables to chaos and equilibration in the quench being studied, finding that local observables are well approximated either due to low entanglement in the global wavefunction or the proximity of local marginal states to the maximally mixed state.

% These findings highlight the challenge of identifying relevant quantum phenomena that remain inaccessible to classical descriptions. Chaotic evolution, while making the classical simulation of the exact many-body state intractable at long times and large system sizes, scrambles information and makes macro-properties more amenable to classical simulation. Understanding the regimes where classical descriptions fail but remain accessible to pre-fault tolerant quantum hardware will help inform the design of future quantum information processors.


==> frontmatter/dedication.tex <==
\textbf{Dedication}

% \noindent
% The dissertation is dedicated to the first nations of New Mexico, including but not limited to the Pueblo, Navajo, and Apache; the homeless humans and animals of New Mexico who deserve the amenities, benefits, dignities, and opportunities that we the privileged enjoy; and to the memory of between 7,043,660 and 33,500,000 human beings who have died, so far, due to the COVID-19 pandemic.

\noindent Dedicated to 
\begin{itemize}
\item the first nations of New Mexico, including but not limited to the Pueblo, Navajo, and Apache; 
\item the homeless humans and animals of New Mexico who deserve the amenities, benefits, dignities, and opportunities that we the privileged enjoy; and 
\item the memory of between 7,043,660 and 33,500,000 human beings who have died, so far, due to the COVID-19 pandemic.
\end{itemize}

==> frontmatter/thanks.tex <==
I do not have adequate words in English, or any other language, to express my gratitude to my advisor, Ivan Deutsch. Ivan took me, a relatively raw hand in quantum information processing with atomic systems, under his wing and nurtured my learning of not only atomic physics and quantum control but also aspects of quantum many-body physics.

Throughout this arduous journey, his remarkable empathy and supportive demeanor have been a beacon of strength, guiding me through both academic challenges and personal struggles. Ivan possesses a rare gift for understanding the complexities of not only the research process but also the human experience. His empathetic approach has fostered an environment where I felt comfortable sharing my uncertainties, fears, and triumphs without hesitation. In moments of self-doubt, he has been a guiding light with his reassurance and perspective, reminding me of my capabilities and the importance of resilience in the face of difficult circumstances. Beyond his scholarly expertise, Ivan has demonstrated an unparalleled commitment to my well-being and success, in a manner that seems too good to be true.

I cannot express sufficient gratitude towards Tameem Albash, for being a mentor and working together in our endeavors in quantum simulation. The range of support I got from Tameem, never ceased to amaze me, from debugging and optimizing the implementation of tensor network algorithms to the physical interpretation of critical exponents. Furthermore, he shared his enthusiasm for using high-performance computing to solve hard scientific problems and nurtured mine. Additionally, I benefited from Tameem's wisdom and penchant for thoroughness in scientific analysis -- I hope to live up to this standard. 

During my Ph.D., I have benefited from close collaboration with experimental colleagues in understanding aspects of ultracold atoms which I could not have imagined, while working on theoretical physics. I am grateful to Grant Biedermann for helping me understand several aspects of experiments with atomic platforms, from the minutiae of Doppler dephasing for adiabatic Rydberg dressing gates to the challenges and considerations in developing a neutral atom quantum information processing platform. 

I am grateful to Michael (Mike) Martin for his perspectives and guidance in thinking about the physical aspects of rapid adiabatic passages and the properties of laser-dressed states of atoms. Thank you to Mike, also for sharing his perspective on the intricacies of developing a neutral atom quantum information processing platform. Finally, the spin echo sequence interleaved with Rydberg dressing passages, which is at the heart of the Mølmer-Sørensen gate for neutral atoms, was designed and implemented by Mike; hence we have colloquially referred to it as the `vanilla Mike gate'.

I am grateful to Akimasa Miyake for guiding me through my journey in studying quantum many-body physics and tensor network methods. Additionally, I benefited from his Graduate Quantum Mechanics and Quantum Computation courses, where I learned a rigorous way of working on problems in quantum mechanics and quantum information science in general. Indeed, I can relate some of my research directions to my lessons in Akimasa's courses.

I am grateful to Pablo Poggi for his invaluable feedback, insightful discussions, and endless encouragement. Pablo has helped my efforts in quantum control, quantum many-body physics, and quantum chaos. Pablo's willingness to lend a listening ear, provide constructive criticism, and offer words of encouragement have significantly enriched the work presented here.

I want to thank Philip Blocher for working together in our quantum simulation endeavors, working through the minutiae of tensor network algorithms for both closed systems, and his deep insights on quantum measurements. My understanding of problems in quantum many-body physics has been enriched by discussions with Jun Takahashi. Jun not only helped me ask the right questions but also taught me to find ways of trying to answer them. My interest in working on these problems was nurtured through long discussions with Jun.

I am grateful to Carlton Caves, Elohim Becerra, Milad Marvian, Susan Atlas for insightful discussions, suggestions, and feedback on my work and presentations. I also want to thank Ivan, Akimasa, Tameem, and Grant for being part of my dissertation committee and helping in the culmination of my Ph.D. work. 

I am grateful for my collaboration with Sivaprasad (Siva) Omanakuttan on the adiabatic Rydberg dressing and nuclear spin qudit and optimal control endeavors. Siva has also been a tremendous colleague to work with and learn from. Fellow Ph.D. students Karthik Chinni and Manuel Muñoz-Arias in Ivan's group and Austin Daniel in Akimasa's group have helped me understand how to approach problems and try to ask appropriate questions. Austin, Karthik, Manuel, and Siva have served as real-time inspirations when I have faced challenges in my research, both through their encouragement and their examples. Our shared endeavors have blossomed into deep lifelong friendships.

During my time at CQuIC, I had the fortune of crossing paths with many students and postdocs. I am grateful to Travis Scholten, for giving me detailed feedback on my first scientific presentation and helping me develop the skills to give effective presentations of my research to technical audiences. I am grateful to Jonathan Gross, Xiaodong Qi, and Travis for their enthusiasm toward developing and teaching skills for classical computation in scientific research. In particular, I am grateful for the CQuIC Summer Computing workshop we conducted together\footnote{https://github.com/CQuIC/summer17-computing-workshop, retrieved on 2024 April 09}. I am grateful for the discussions, and learning efforts with Ezad Shojaee, Xiaodong Qi, and Gopikrishan Muraleedharan in Ivan's group. I am grateful to Anirban Chowdhury for helping me think algorithmically about quantum computation, which has deeply benefited my approach to thinking about quantum information science. I am also grateful to Adrian Chapman, Andrew Zhao, Christopher Jackson, Jacob Miller, Julie Campos, Ninnat Dangniam, Rafael Alexander, Sam Slezak, and Sayonee Ray, for helping me grow as a researcher in quantum information science.

I want to thank Adrian Chapman, Adrian Orozco, Alex Fisher, Andrew Ferdinand, Andrew Forbes, Andrew Zhao, Anirban Chowdhury, Ben Morrison, Benjamin Anker, Benjamin Corbett, Bibek Pokharel, Christopher Jackson, Cole Kelson-Packer, Cole Maurer, Connor Smith, Cunlu Zhou, Evan Borras, Ezad Shojaee, Gopikrishan Muraleedharan, Hariprasad Madathil, Ivy Gunther, Jacob Miller, Jalan Ziyad, John DeBrota, Jonathan Gross, Juan Gonzalez de Mendoza, Jun Takahashi, Kaleb Campbell, Karthik, Leeseok Kim, Manuel, Marco Rodriguez Garcia, Matt Chao, Mitchell Brickson, Mohammad Alhejji, Mohsin Raza, Namitha Pradeep, Ninnat Dangniam, Pablo Poggi, Philip Blocher, Rafael Alexander, Robert Kramer, Sam Slezak, Sayonee Ray, Siva, Spencer Dimitroff, Srinidhi Pawar, Sujeet Pani, Travis Scholten, Tyler Thurtell, Tzula Propp, Vikas Buchemmavari, Xiaodong Qi, for their presence at CQuIC, for my hallway conversations with them on a variety of topics, which helped me learn several things and also made my time here so rewarding.

I am grateful to the National Science Foundation (NSF), the Air Force Office of Scientific Research (AFOSR), and the Quantum Systems Accelerator (QSA) for supporting our research endeavors. I also want to thank the developers of open-source software libraries ITensor, ITensors.jl, QuantumOptics.jl, Quimb, QuTiP, TenPy. As a computer programmer at heart, I have learned many things from reading their source code which I could have not learned elsewhere.

During the first few semesters of the Ph.D. program, I had the privilege of teaching introductory calculus-based Physics Laboratory courses, under the guidance of Mickey Odom. Teaching these courses was an extremely rewarding and enjoyable experience. Thank you to Mickey, for both structuring the laboratory and experiences to be enjoyable both for the students and instructors. Thank you to Mickey, also, for nurturing our abilities to teach concepts to students with empathy.

I am extremely grateful to Alisa Gibson, for helping me navigate the formalities and logistics of the Ph.D. program in Physics at UNM. From my initial questions about the application requirements for the program to the details of crossing every hurdle through the program, I could not have done without Alisa. Thank you to Steven Bishop, for taking over the reins and helping me navigate the program after Alisa's retirement.

Thank you to Gloria Cordova, Dwight Zier, and David Tenen for helping with the affairs of CQuIC. From arranging conference registrations and travel to procuring computer hardware and other materials, I would not have been able to be where I am without their support.

I am grateful to my healthcare providers and other staff at the UNM Student Health and Counseling (SHAC). They have helped me through my health challenges throughout my Ph.D. at the UNM.

As an international student, I recognize the significant privilege I enjoy in the circumstances and logistics of my move to the USA. In contrast with people come to the USA under extremely difficult and precarious circumstances, sometimes by foot, I was fortunate to arrive in this country by plane and with offers of Teaching and Research Assistantships providing financial support for my life expenses. At the same time, I know the process of moving one's entire life to a foreign country with different a culture and different legal processes to pursue a graduate degree, is a tantamount challenge. I am grateful to the Graduate Education Office (GEO) for helping me navigate the intricacies of my student visa and other formalities of living in the USA. I am also grateful to International Students Inc. (ISI) Albuquerque for their support of international students in New Mexico. ISI has helped us in many ways, from arranging host families for incoming international students to helping with trips in house hunting, running errands, buying and transporting items, and organizing home groups with welcoming and homely environments. Moreover, I am grateful to all the different extraordinary people I have had the opportunity to meet during my time in New Mexico, who have been extremely friendly and supportive in my moments of need.

I also want to thank the friends I made during the Ph.D. -- Adrian Orozco, Akram Etemadi Amin, Alexandre Mills, Andrew Ferdinand, Anthony Demme, Bibek Pokharel, Jaimie Stephens, Kaleb Campbell, Karishma Bansal, Kishore Vakamudi, Matt Chow, Matt Curry, Matt Pillion, Maziar Saleh Ziabari, Mitchell Brickson, Nathan Lysne, Nazanin Mosavian, Satomi Sugaya. You have made my experience highly enjoyable and rewarding, and given me friendships and memories to cherish for the rest of my life.

My dear friends who supported the efforts of United Graduate Workers of UNM (UGW), Anna Rose, Dominic Oddo, Duncan McGraw, Emma Mincks, Ian Birdwell, Julie Hayes, Katie Despeaux, Kim Lawson, Ramona Malczynski, Samantha Cooney, thank you for the solidarity, support, friendship and your dedication to make things better for everyone.

I would not have gotten here without the unremitting support of my beloved friends Abhik, Amy, Ananta, Bhaswar, Jyotiprakash, Mihir, Pratik, Yash. I am grateful to them for taking care of me and for their patience and understanding. Their unwavering support and belief in my abilities have been a constant source of strength. I would also like to extend my appreciation to all my friends who may not be named here but have nonetheless played a significant role in shaping my academic journey. Their friendship, camaraderie, and shared experiences have made this journey memorable and meaningful. They have been the cornerstone of my success, and I am forever grateful for their presence in my life. Special thank you to Yash for holding my hands when I have faced difficulties during the arduous Ph.D. journey.

Thank you to my American family Choon, Robert and Chan, who accepted me into their family from the moment I arrived in the USA and made me feel as much at home with them as I have ever before, through their warmth, hospitality, and unwavering support. Their kindness, generosity, and genuine interest in my well-being created an environment conducive to academic pursuits and personal growth. I am truly grateful for the countless meals, conversations, and cultural exchanges that enriched my experience and made my time in Albuquerque both comfortable and memorable.

Thank you to my partner Šárka, her parents Lynne and Ed. I am very grateful to be welcomed me into the family with open arms and for their unwavering support and encouragement throughout this journey. Their kindness, guidance, and words of wisdom have been a source of strength and inspiration. Thank you to my mother Tara, and father Gautam for supporting my dreams of pursuing a career in scientific research. Their unconditional love, unremitting support, and belief in my potential have been the guiding lights of my life. Their sacrifices, encouragement, and words of wisdom have shaped me into the person I am today, and I am forever indebted to them for their unwavering love and support. My father, Gautam, was my initial inspiration to be curious, ask questions, and work towards contributing to scientific research. It is unfortunate that he passed away and was unable to see me complete my Ph.D. 

In addition to humans, I am extremely grateful to canine individuals Bob, Lola, Orion, Winnie, Yang, Zoom, and feline individuals Axel, Bo, Cleo, Hagrid, Harvey, Laszlo, Molly, Penny, Schrödi, who have given me unconditional love and affection that I cannot describe in human terms.

Finally, I want to end with the UNM Indigenous Peoples' Land and Territory Acknowledgement

\begin{quote}
    Founded in 1889, the University of New Mexico sits on the traditional homelands of the Pueblo of Sandia. The original peoples of New Mexico – Pueblo, Navajo, and Apache – since time immemorial, have deep connections to the land and have made significant contributions to the broader community statewide. We honor the land itself and those who remain stewards of this land throughout the generations and also acknowledge our committed relationship to Indigenous peoples. 
    We gratefully recognize our history.
\end{quote}

and with UNM's Statement Acknowledging the Labor and Sacrifices of Black Americans\footnote{https://diverse.unm.edu/about-dei-at-unm/land-labor-acknowledgement.html, retrieved on 2024 April 09}

\begin{quote}
At UNM, we respectfully acknowledge the traumatic history of forced labor of Black Americans who have advanced our country. We are indebted to the enslaved and exploited African Americans who established our U.S. infrastructure and economy, advanced civil rights, and continue to influence popular culture. We are obligated to continuously recognize historic and current systemic oppression and injustices placed on Black Americans. We are grateful to their ancestors; for without them we would not be where we are today. - (Fall 2022 FYEX 1110 Black Minds Matter Class)
\end{quote}

Science is a social endeavor, and findings result from collective efforts like discussion with colleagues and reading and interpreting literature, and due to the support of others both within and outside the scientific community. In this spirit, I will use the \textit{pluralis modestati} form `we' throughout the dissertation.

\noindent
\begin{tabular}{l}
\\
\\
Anupam Mitra
\\
2024 April 14
\\
Albuquerque, NM, USA
\end{tabular}
